A Characterization of Approximability for Biased CSPs

A $\mu$-biased Max-CSP instance with predicate $\psi:\{0,1\}^r \to \{0,1\}$ is an instance of Constraint Satisfaction Problem (CSP) where the objective is to find a labeling of relative weight at most $\mu$ which satisfies the maximum fraction of constraints. Biased CSPs are versatile and express several well studied problems such as Densest-$k$-Sub(Hyper)graph and SmallSetExpansion. In this work, we explore the role played by the bias parameter $\mu$ on the approximability of biased CSPs. We show that the approximability of such CSPs can be characterized (up to loss of factors of arity $r$) using the bias-approximation curve of Densest-$k$-SubHypergraph (DkSH). In particular, this gives a tight characterization of predicates which admit approximation guarantees that are independent of the bias parameter $\mu$. Motivated by the above, we give new approximation and hardness results for DkSH. In particular, assuming the Small Set Expansion Hypothesis (SSEH), we show that DkSH with arity $r$ and $k = \mu n$ is NP-hard to approximate to a factor of $\Omega(r^3\mu^{r-1}\log(1/\mu))$ for every $r \geq 2$ and $\mu < 2^{-r}$. We also give a $O(\mu^{r-1}\log(1/\mu))$-approximation algorithm for the same setting. Our upper and lower bounds are tight up to constant factors, when the arity $r$ is a constant, and in particular, imply the first tight approximation bounds for the Densest-$k$-Subgraph problem in the linear bias regime. Furthermore, using the above characterization, our results also imply matching algorithms and hardness for every biased CSP of constant arity.

==> algo-redn.tex <==
\section{Algorithm for the Weighted Setting}

The main result of this section is the following theorem.



The key component required for establishing Theorem \ref{lem:at-most-0} is the following: we will show that for any $\beta \in \{0,1\}^r$, the corresponding single string predicate admits $\alpha^{\sf uw}_{(\mu)}(\dksh_{\|\beta\|_0})$-approximation (Lemma \ref{lem:at-most}). Using the above, we can prove Theorem \ref{lem:at-most-0} in the following way. Firstly, we will show that without loss of generality, there exists a labeling of weight at most $\mu$ which satisfies a significant fraction of edges using patterns from $\cM_\psi$, in comparison to the fraction of edges satisfied by the optimal labeling of weight at most $\mu$. Furthermore, by an averaging argument, at least one of the single string predicates $\beta^* \in \cM_{\psi}$ contributes at least $2^{-r}$-fraction of satisfied edges. Therefore, using Lemma \ref{lem:at-most} on the instance with the single string predicate $\psi_{\beta^*}$ yields would yield a labeling of weight at most $\mu$ which satisfies a significant fraction of edges (where the loss due to approximation will be due to the weight of the string $\|\beta\|_0$).





\subsection{Auxiliary Lemmas}







==> completeness-lift.tex <==
\section{Completeness}

Suppose $G$ is a YES instance. Then there exists $S \subset V$ such that ${\sf Vol}(S) = \delta$ and $\phi_G(S) \leq \epsilon$. As is usual, we define the map $i^* : V^R \times \{\bot,\top\}^R \to [R]$ as follows. For every $(A,z) \in V^R \times \{\bot,\top\}^R$, define the set $\Pi(A,z) := \{i \in [R]| (A(i),z(i)) \in S \times \{\top\}\}$. Then we assign $i^*(A,z)$ as follows: if $|\Pi(A,z)| = 1$, then we assign $i^*(A,z) = i$ where $i$ is the element contained in $\Pi(A,z)$, otherwise we assign $i^*(A,z) \in [R]$ arbitrarily. Finally, for every $(A,z) \in V^R \times \{\bot,\top\}^R$, we assign the dictator function $f_{A,z} := \chi_{i^*(A,z)}$.

Now we analyze the probability of the test accepting this assignment. Towards that, fix a hyperedge $e = [r] \in E$, let $\cD_e$ denote the test distribution conditioned on the choice of $e$. We shall also find it convenient to define the events:
\begin{gather*}
\cE:= \Big\{ \forall \ j \in e, \  {\theta}_j(i^*(A,z)) = 1 \Big\} \wedge \Big\{|\Pi(A,z)| = 1\}  \\
\cE':= \Big\{\forall \ j \in e, \  \Pi(B'_j,z'_j) = \Pi(A,z)	\Big\} 
\end{gather*} 
Note that 
\begin{equation}			\label{eqn:e-prob}
\Pr_{\cD_e} \big[\cE\big] = \Pr{(A,z)}\big[|\Pi(A,z)|= 1\big] \Pr_{X_e \sim \nu_e}\big[X_e = {\bf 1}_e\big] = e^{-1} \cdot \Pr_{X_e \sim \nu_e}\big[X_e = {\bf 1}_e\big]
\end{equation}

Now we state the analogous version of Lemma \ref{lem:match-ix} from Section \ref{sec:dksh-comp}.

\begin{lemma} 				\label{lem:i-match}
	Under the test distribution, for any hyperedge $e \in E_{\rm gap}$ of arity $r$ we have 
	\[
	\Pr_{(B'_j,x'_j,z'_j)_{j \in e}} \Big[ \cE \wedge \cE' \wedge \big\{|\Pi(A,z)| = 1\}\Big] \geq  p_e \cdot e^{-Cr - 1} - r\eta, 
	\]
	where $C > 0$ is an absolute constant.
\end{lemma}
\begin{proof}
	This directly follows from Lemma \ref{lem:match-ix}. Observe that the events $\cE$,$\cE'$ and $|\Pi(A,z)| = 1$, involve the variables $A,\{B'_j\}_{j \in e},z,\{z'_j\}_{j \in e},\{{\theta}_j\}_{j \in [r]}$. We claim  that the joint distribution of these variables under the distribution from Test \ref{fig:test-1} is identical to the distribution from Figure \ref{fig:dksh-test} instantiated with $\rho = \sqrt{p_e}$ and $e = [r]$. Indeed, under both tests $A,\{B_j\}_{j \in e}$ are identically distributed, and are sampled independent of the $z$ and $\theta$ variables. Furthermore, for every $j \in [R]$, ${\theta}_1(j),\ldots,{\theta}_r(j)$ is identically generated using the distribution $\cA_{r,\rho}$ with $\rho = \sqrt{p_e}$, and $\hat{\theta}_i$ are $1 - \eta$ correlated copies of $\theta_i$ under both distributions. Again, for a fixing of ${\theta}_1,\ldots,{\theta}_r$, the variables $z'_1,\ldots,z'_r$ are generated identically, which also implies that $B'_1,\ldots,B'_r$ are identically distributed, thus establishing the claimed equivalence.
	
	In summary, the probability of any event determined these variables will be identical under the two distributions. Hence using Lemma \ref{lem:match-ix} we get
	\begin{align}
		&\Pr_{(B'_j,x'_j,z'_j)_{j \in e}} \Big[ \cE \wedge \Big\{\forall j \in [r], \theta_j(i^*(A,z)) = 1\Big\} \wedge \big\{|\Pi(A,z)| = 1\}\Big] \\
		& \geq \Pr_{(B'_j,x'_j,z'_j)_{j \in e}} \Big[ \cE \wedge \Big\{\forall j \in [r], \hat{\theta}_j(i^*(A,z)) = 1\Big\} \wedge \big\{|\Pi(A,z)| = 1\}\Big] - r\eta \\
		& \geq  p_e \cdot e^{-C r - 1}- r\eta. 
	\end{align}
	\end{proof}

Denote the event $\cE_1 := \cE \wedge \cE' \wedge \big\{|\Pi(A,z)| = 1\}$. Using the above, we can bound the probability of the test accepting (conditioned on the choice of $e = [r] \in E$):

\begin{align*}
	\Pr_{\cD_e}\Big[\mbox{ Test Accepts }\Big]
	& = \Pr_{(B'_j,x'_j,z'_j)_{j \in [r]}} \Big[\forall j \in [r], \ f(B'_j,x'_j,z'_j) = 1\Big] \\
	& \overset{1}{=} \Pr_{(B'_j,x'_j,z'_j)_{j \in [r]}} \Big[\forall j \in [r], \ x'_j(i^*(B'_j,z'_j)) = 1\Big] \\
	& \geq \Pr_{(B_j,x_j,z_j)_{j \in [r]}}\big[\cE_1\big] \Pr_{(B'_j,x'_j,z'_j)_{j \in [r]}} 
	\Big[\forall j \in [r], \  {x}'_j(i^*(B'_j,z'_j)) = 1 \Big| \cE_1\Big]\\
	& \overset{2}{\geq} \left(p_e \cdot e^{-Cr - 1}  - r\eta \right)\cdot \Pr_{(B'_j,x'_j,z'_j)_{j \in [r]}} \Big[\forall j \in [r], \  {x}'_j(i^*(B'_j,z'_j)) = 1 \Big| \cE_1\Big]\\
	& = \overset{3}{\geq} \left(p_e \cdot e^{-Cr - 1}  - r\eta \right)\cdot \Pr_{(B'_j,x'_j,z'_j)_{j \in [r]}} \Big[\forall j \in [r], \  \tilde{x}_j(i^*(B'_j,z'_j)) = 1 \Big| \cE_1\Big]\\
	& \overset{4}{\geq}  \left(p_e \cdot e^{-Cr - 1} p_e - r \eta\right) \cdot \Pr_{(B'_j,x'_j,z'_j)_{j \in [r]}} \Big[\forall j \in [r], \  {x}_j(i^*(A,z)) = 1 \Big| \cE_1\Big] - r\eta\\
	& \overset{5}{\geq}  p_e \cdot e^{-Cr - 1}  - 2r\eta.			\label{eqn:lift-comp}
\end{align*}
Here, step $1$ is the definition of $f$. Step $2$ bounds the first term using Lemma \ref{lem:i-match}. In step $3$, we observe that conditioned on $\cE_1$, for every $j \in [d]$, we have $|\Pi(B'_j,z'_j)| = 1$, which in turn implies that $z'_j(i^*(B'_j,z'_j)) = \top$ (using the definition of $i^*$) and hence $\tilde{x}_j(i^*(B'_j,z'_j)) = x'_j(i^*(B'_j,z'_j))$ (using the definition of $M_{z'_i})$ operator). Step $4$ again uses $i^*(B'_j,z'_j) = i^*(A,z)$ conditioned on the event $\cE$, and the final step follows using $x(i^*(A,z)) = {\bf 1}_r$ is again implied by $\cE_1$.

Now, averaging over the choice of $e \in E_{\rm gap}$ and applying \eqref{eqn:lift-comp} for each choice of edge we get that:
\[
\Ex_{e \sim E_{\rm gap}}\Pr_{\cD_e}\Big[\mbox{ Test Accepts }\Big]
\gtrsim e^{-Cr} \Ex_{e \sim E_{\rm gap}} \left[\Pr_{X_e \sim \nu_e} \Big[X_e = \mathbbm{1}_e \Big]\right] - 2r\eta \geq e^{-Cr}  \cdot {\sf Sdp}(G_{\rm gap}) - 2r\eta.
\]


==> csp-prelims.tex <==
\section{Preliminaries for Hardness Results}

\subsection{Fourier Analysis}

\subsection{Invariance Principles}

We shall need the following Invariance Principle from [] which shows that distributions with matching covariance structure fool functions with no influential coordinates.

\begin{theorem}					\label{thm:clt2}
	Let $\cX := (\cX_1,\ldots,\cX_t)$ be an independent sequence of ensembles on a finite probability space $(\prod_{i \in [t]} \Omega_i,\prod_{i \in [t]} \mu_i)$ such that the probability of each atom is at least $\alpha$ i.e,. $\Pr_{\mu_i}\left[\cX_i = x\right] \geq \alpha$ for every $x \in \Omega_i$. Let $Q$ be a $k$-dimensional multilinear polynomial such that ${\rm Var}\left[Q_j(\cX)\right] \leq 1$ and ${\rm Var}\left[Q^{>p}(\cX)\right] \leq (1 - \eta)^{2p}$, for $p = O(\log(1/\tau)/\log(1/\alpha))$. Furthermore, let $\max_{i} \Inf{i}{Q_j} \leq \tau$ for every $i \in [k]$. Finally, let $\Psi:\mathbbm{R}^k \to \mathbbm{R}$ be $L$-lipschitz continuous. Then, 
	\[
	\left|\Ex_{\cX}\left[\psi\left(Q(\cX)\right)\right] - \Ex_{\cY}\left[\psi\left(Q(\cY)\right)\right]\right| \leq C_kL\tau^{\eta/\log(1/\alpha)}
	\]
	where $\cY$ is an independent sequence of ensembles with matching covariance structure as $\cX$, and $C_k$ is a constant depending only on $k$.
\end{theorem}

We shall need the following variant of Invariance which can be used to pass on from a pairwise independent distribution to a fully independent distribution with up to matching second moments.

\begin{theorem}				   \label{thm:clt1}
	Let $(\Omega,\mu)$ be a finite probability space over $\Omega:= \prod^{k}_{i = 1} \Omega_i$ with the following properties:
	\begin{itemize}
		\item $\mu$ is pairwise independent.
		\item For every $i \in [k]$ and $b_i \in \Omega_i$ we have $\mu_i(b_i) > \alpha$.
		\item $\rho(\Omega_1,\ldots,\Omega_k) < 1$.
	\end{itemize}
	Then for every $\nu > 0$, there exists $\tau > 0$ and $d> 0$ such that the following holds for all $t$. Let $f_1,\ldots,f_k$ be functions $f_i:\Omega^t_i \to [0,1]$ satisfying
	\[
	\max_{j \in [k]}\max_{\ell \in [t]} \Inf{\ell}{T_{1 - \eta} f_j} \leq \tau.
	\] 
	Then
	\[
	\left|\Ex_{\left(\theta_i\right)^k_{i = 1} \sim \Omega}\left[\prod_{j \in [k]}T_{1 - \eta}f_j(\theta^{(1)}_{j},\ldots,\theta^{(t)}_{j})\right]
	- \prod_{j \in [k]} \Ex_{\left(\theta_i\right)^k_{i = 1} \sim \Omega}\left[T_{1 - \eta}f_j(\theta^{(1)}_{j},\ldots,\theta^{(t)}_{j})\right]
	\right| \leq \tau^{(\eta)/\log(1/\alpha)}.
	\]
\end{theorem}







==> gen-pred.tex <==
\section{Generalizing to Predicates with Negations}			\label{sec:cond-gen}

Theorems \ref{thm:pred-cond} and \ref{thm:pred-approx} readily admit extensions to the more general setting where variables can appear with negations as input the predicate. We introduce some additional notation towards stating our results. Given a Boolean string $x \in \{0,1\}^r$ and $r$-bit pattern string $\pi \in \{\pm 1\}^r$, we use $\pi\circ x$ to denote the corresponding string $x$ negated with respect to pattern $\pi$ i.e.,
\[
\Big(\pi \circ x\Big)(i)
\begin{cases}
	x(i) & \mbox{ if } \pi(i) = 1 \\
	\bar{x}(i) & \mbox{ if } 	\pi(i) = -1
\end{cases} 
\]
Furthermore, given a $r$-ary Boolean predicate $\psi:\{0,1\}^r \to \{0,1\}$, and a negation pattern $\pi$, we use $\pi(\psi) $ to denote the predicate corresponding to the map $x \mapsto \psi\big(\pi \circ x\big)$. Finally, here we denote $\mcsp$ instances as $\Psi(E,V,\{\pi_e\}_{e \in E})$ where $V$ and $E$ are still the vertex and edge set of the constraint graph, and for every edge $e \in E$, $\pi_e \in \{\pm 1\}^r$ identifies the negation pattern for edge $e$. Finally, for predicate $\psi$, let $\alpha^{\rm gen}_{(\mu)}$ be the optimal approximation factor achievable for $\mcsp$s on predicate $\psi$ with negations. We are now ready to state our extensions to Theorems \ref{thm:pred-cond} and \ref{thm:pred-approx} to this setting. .

\begin{theorem}				\label{thm:pred-cond-gen}
	The following holds assuming SSEH. A predicate $\psi:\{0,1\}^r \to \{0,1\}$ is bias independent under negations if and only if the following holds: for every negation pattern $\pi \in \{\pm 1\}^r$ we have $\cM_{\pi(\psi)} \cup \cM_{\pi(\bar{\psi})} \subseteq \cS_{\leq 1}$.
\end{theorem}
	
		
\begin{theorem}				\label{thm:pred-approx-gen}
	For every $r \geq 2$, for any $\mu \in (0,1)$, the following holds for any predicate $\psi:\{0,1\}^r \to \{0,1\}$:
	\[
	\alpha^{\rm gen}_{(\mu)}(\psi) \asymp_r \min_{\pi \in \{\pm 1\}^r}\min\left\{\min_{\beta \in \cM_{\pi(\psi)}} \alpha_{(\mu)}\left({\sf D}k{\sf SH}_{{\|\beta\|_0}}\right),\min_{\beta \in \cM_{\pi(\bar{\psi})}} \alpha_{(1-\mu)}\left({\sf D}k{\sf SH}_{{\|\beta\|_0}}\right)\right\},
	\]
	where $\|\cdot\|_0$ denotes the Hamming weight of a string, and $\asymp_r$ is used to denote that the two sides are equal up to multiplicative factors depending on $r$.
\end{theorem} 

The above theorems again follow using Lemmas \ref{lem:pred-apprx}, \ref{lem:pred-hard} and \ref{lem:pred-apprx2}, we prove them formally below.

\subsection{Proof of Theorem \ref{thm:pred-cond-gen}}

For a predicate $\psi:\{0,1\}^r \to \{0,1\}$, define $w(\psi)$ as 
\begin{equation}			\label{eqn:w-def}
w(\psi) := \max_{\pi  \in \{\pm 1\}^r} \max_{\beta \in \cM_{\pi(\psi)} \cup \cM_{\pi(\bar{\psi})}} \|\beta\|_0
\end{equation}
Now we consider the two cases.

{\bf Case (i)}: Suppose $w(\psi) \leq 1$. In this case, as before, we can show that there exists a $2^{-3r}/(er)$-approximation algorithm for $\mcsp(\psi)$ with negations, which is the following simple extension of the algorithm from Lemma \ref{lem:pred-apprx}: 

	\begin{algorithm}[ht!]
	\SetAlgoLined
	\KwIn{$\mu$-biased instance $\Psi_{(\mu)}(V,E,\{\pi_e\}_{e \in E})$} 
	If $\mu \in (0,1/2)$, set $\psi_1 \gets \psi$ and $\mu_1 \gets \mu$, otherwise let $\psi_1 \gets \bar{\psi}$ and $\mu_1 \gets 1 - \mu$\;
	\For{$\pi \in \{\pm 1\}^r$}
	{
		Let $E_\pi \subseteq E$ be the subset of edges for which $\pi_e : = \pi$\;
		Run Algorithm \ref{alg:approx-pred} on $\Psi_\pi := \Psi(V,E_\pi)$ with predicate $\pi(\psi_1)$ with bias constraint $\mu_1$\; 
		Let $\sigma_\pi$ denote the corresponding $\mu_1$-biased labeling returned by the algorithm\;
	}
	Let $\sigma:V \to \{0,1\}$ be the labeling satisfying the largest number of constraints i.e.,
	\[
	\sigma = \argmax_{\pi \in \{\pm 1\}^r} \left|\Big\{e \in E_\pi~\Big|~\psi_1(\sigma_\pi(e)) = 1 \Big\} \right|.
	\]
	\If{$\mu \leq 1/2$}
	{
		Ouput labeling $\sigma$
	}
	\Else{
		Ouput labeling $\bar{\sigma}$.
	}
	\caption{Approx-Pred-Gen}
	\label{alg:approx-pred-gen}
	\end{algorithm}	

We analyze the above algorithm. Consider the case $\mu\leq 1/2$ (the other cases follows similarly). Then note that $\psi_1 = \psi$ and $\mu_1 = \mu$.
Let $\sigma':V \to \{0,1\}$ be the optimal $\mu$-biased labeling for $\Psi$. Let $E' \subset E$ be the subset of constraints satisfied by $\sigma'$, and for every $\pi \in \{\pm 1\}^r$, let $E'_\pi := E \cap E_\pi$. Then, by averaging, there exists negation pattern $\pi^* \in \{\pm 1\}^r$ such that $|E'_{\pi^*}| \geq 2^{-r}|E'|$. This in turn implies that 
\begin{equation}			\label{eqn:opt-pi}
{\sf Opt}_{(\mu)}(\Psi_{\pi^*}; \pi^*(\psi)) \geq 2^{-r} \cdot |E'|. 
\end{equation}
Therefore, using the guarantee of Lemma \ref{lem:pred-apprx}, we know that Algorithm \ref{alg:approx-pred} returns a $\mu$-biased labeling $\sigma_{\pi*}$ with the guarantee
\[
{\sf Val}_{\sigma_{\pi*}}\left(\Psi_{\pi*}\right) \geq \frac{2^{-2r}}{er} \cdot {\rm Opt}_{(\mu)}(\Psi_{\pi^*};\pi^*(\psi)) \geq \frac{2^{-3r}}{er} \cdot |E'| 
\]
where the last step follows from \eqref{eqn:opt-pi}. Furthermore, since $E_{\pi^*} \subset E$, it follows that $\sigma_{\pi^*}$ would also satisfy at least $2^{-3r}|E'|/(er)$-constraints of $E$. Since the algorithm outputs the best among all labelings $\sigma_\pi$, it would output a labeling which satisfies at least $2^{-3r}|E'|/(er)$-constraints, which establishes the approximation guarantee of Algorithm \ref{alg:approx-pred-gen}, thus concluding this case.

{\bf Case (ii)}: Suppose $w(\psi) > 1$. Then there exists $\pi \in \{\pm 1\}^r$ such that 
\[
\cM_{\pi(\psi)} \cup \cM_{\pi(\bar{\psi})} \not\subset \cS_0 \cup \cS_1.
\]
Then using Theorem \ref{thm:pred-cond} we know that 
\[
\inf_{\mu \in (0,1)} \alpha_{(\mu)}(\pi(\psi)) = 0.
\]
Furthermore, by definition we have $\alpha^{\rm gen}_{(\mu)}(\pi(\psi)) \leq \alpha_{(\mu)}(\psi)$, the claim follows.

\subsection{Proof of Theorem \ref{thm:pred-approx-gen}}
Let 
\[
\hat{\pi} := \argmin_{\pi \in \{\pm 1\}^r}\min\left\{\min_{\beta \in \cM_{\pi(\psi)}} \alpha_{(\mu)}\left({\sf D}k{\sf SH}_{{\|\beta\|_0}}\right), \min_{\beta \in \cM_{\pi(\bar{\psi})}} \alpha_{(1-\mu)}\left({\sf D}k{\sf SH}_{{\|\beta\|_0}}\right) \right\}.
\]
Since $\mcsp(\Psi)$~instances on predicate $\psi$ with negations contain $\mu$-biased $\mcsp$ instances with predicate $\hat{\pi}(\psi)$, using Theorem \ref{thm:pred-approx} we immediately have 
\[
\alpha^{\rm gen}_{(\mu)}(\psi) \leq \alpha_{(\mu)}\left(\hat{\pi}(\psi)\right) \lesssim_r 
\min\left\{\min_{\beta \in \cM_{\hat{\pi}(\psi)}} \alpha_{(\mu)}\left({\sf D}k{\sf SH}_{{\|\beta\|_0}}\right), \min_{\beta \in \cM_{\hat{\pi}(\bar{\psi})}} \alpha_{(1-\mu)}\left({\sf D}k{\sf SH}_{{\|\beta\|_0}}\right) \right\}
\]
which, along with the definition of $\hat{\pi}$ establishes the $\lesssim_r$ direction. For the $\gtrsim_r$ direction, again consider the following extension of Algorithm \ref{alg:Gen-pred}:

	\begin{algorithm}[ht!]
	\SetAlgoLined
	\KwIn{$\mu$-biased instance $\Psi_{(\mu)}(V,E,\{\pi_e\}_{e \in E})$} 
	If $\mu \in (0,1/2)$, set $\psi_1 \gets \psi$ and $\mu_1 \gets \mu$, otherwise set $\psi_1 \gets \bar{\psi}$ and $\mu_1 \gets \mu$\;
	\For{$\pi \in \{\pm 1\}^r$}
	{
		Let $E_\pi \subset E$ be the subset of edges for which $\pi_e : = \pi$\;
		Run Algorithm \ref{alg:rank-bisect} on $\Psi_\pi := \Psi(V,E_\pi)$ with predicate $\pi(\psi_1)$ with bias constraint $\mu_1$\; 
		Let $\sigma_\pi$ denote the corresponding $\mu_1$-biased labeling returned by the algorithm\;
	}
	Let $\sigma:V \to \{0,1\}$ be the labeling satisfying the largest number of constraints i.e.,
	\[
	\sigma = \argmax_{\pi \in \{\pm 1\}^r}\left|\Big\{e \in E_\pi~\Big|~\psi_1(\sigma_\pi(e)) = 1 \Big\} \right|.
	\]
	\If{$\mu \leq 1/2$}{Output labeling $\sigma$\;}
	\Else{Output labeling $\bar{\sigma}$\;}.
	\caption{Approx-Pred-Gen-I}
	\label{alg:rank-bisect1}
	\end{algorithm} 

The analysis of the algorithm proceeds along the lines of Algorithm \ref{alg:approx-pred-gen}. Again we consider the case $\mu \in (0,1/2)$ (the $\mu \in [1/2,1)$ case will follow using identical arguments). Then note that the algorithm sets $\mu_1 = \mu$ and $\psi_1 = \psi$. Using arguments similar to Theorem \ref{thm:pred-cond-gen}, we can establish that there exists a negation pattern $\pi^* \in \{\pm 1\}^r$ for which 
\[
{\sf Opt}_{(\mu)}(\Psi_{\pi^*}) \geq 2^{-r} {\sf Opt}_{(\mu)}(\Psi).
\] 
Then from Lemma \ref{lem:pred-apprx2}, we know that running Algorithm \ref{alg:rank-bisect1} on $\Psi_{\pi^*}$ will return a $\mu$-biased labeling $\sigma_{\pi^*}$ which satisfies at least $\alpha_{\pi^*} \cdot 2^{-r} {\sf Opt}_{(\mu)}(\Psi)$ constraints where 
\[
\alpha_{\pi^*} \asymp_r \min\left\{\min_{\beta \in \cM_{\pi^*(\psi)}} \alpha_{(\mu)}\left(\dksh_{\|\beta\|_0}\right),
\min_{\beta \in \cM_{\pi^*(\bar{\psi})}} \alpha_{(1-\mu)}\left(\dksh_{\|\beta\|_0}\right)
\right\}. 
\] 
Since Algorithm \ref{alg:rank-bisect1} returns the best labeling among $\{\sigma_\pi\}_\pi$, it follows that the labeling $\sigma$ satisfies at least $2^{-r} \alpha_{\pi^*} \cdot {\sf Opt}_{(\mu)}(\Psi)$ constraints. Finally, since the definition of $\alpha_{\pi*}$ implies that 
\[
\alpha_{\pi^*} \gtrsim_r \min_{\pi \in \{\pm 1\}^r}\min\left\{\min_{\beta \in \cM_{\pi(\psi)}} \alpha_{(\mu)}\left(\dksh_{\|\beta\|_0}\right),
\min_{\beta \in \cM_{\pi(\bar{\psi})}} \alpha_{(1-\mu)}\left(\dksh_{\|\beta\|_0}\right)\right\}
\]
this establishes the $\gtrsim_r$ direction.



